Eliciting the Double-edged Impact of Digitalisation: a Case Study in Rural Areas

Designing systems that account for sustainability concerns demands for a better understanding of the \textit{impact} that digital technology interventions can have on a certain socio-technical context. However, limited studies are available about the elicitation of impact-related information from stakeholders, and strategies are particularly needed to elicit possible long-term effects, including \textit{negative} ones, that go beyond the planned system goals. This paper reports a case study about the impact of digitalisation in remote mountain areas, in the context of a system for ordinary land management and hydro-geological risk control. The elicitation process was based on interviews and workshops. In the initial phase, past and present impacts were identified. In a second phase, future impacts were forecasted through the discussion of two alternative scenarios: a dystopic, technology-intensive one, and a technology-balanced one. The approach was particularly effective in identifying negative impacts. Among them, we highlight the higher stress due to the excess of connectivity, the partial reduction of decision-making abilities, and the risk of marginalisation for certain types of stakeholders. The study posits that before the elicitation of system goals, requirements engineers need to identify the socio-economic impacts of ICT technologies included in the system, as negative effects need to be properly mitigated. Our study contributes to the literature with: a set of impacts specific to the case, which can apply to similar contexts; an effective approach for impact elicitation; and a list of lessons learned from the experience.

==> sections/general.tex <==
\paragraph*{General Abstract}
Society is changing at a rapid pace, with digitalisation transforming businesses, public services and communities. Though technology can help to achieve greater efficiency, it can also have negative effects from a socio-economic viewpoint. Indeed, digitalisation can create winners, but also losers, especially among those subjects who cannot cope with the change, or at least not fast enough. In this study, we investigate positive and negative impacts of digitalisation in a real-world context. We interview a rural community involved in the control of hydro-geological risk through the monitoring and maintenance of rivers and streams. With the advent of sensors, mobile communication, drones, and other technologies, the activities of the community have seen a radical change in the last ten years. The participants highlight that the main benefits of digitalisation are the better control of their process of monitoring and maintenance, and the improved communication, which allows quicker intervention. Negative impacts include: higher stress due to the excess of connectivity; greater distraction of workers due to the intensive usage of mobile apps; 
%the partial reduction of decision-making abilities; 
the loss of control in critical situations, as technology does not function in case of unexpected weather phenomena, when hydro-geological risk becomes higher. The limits and downsides of digitalisation are not jeopardising its benefits, but should be taken into account when introducing novel technologies in existing contexts and processes.
%, especially when they aim to replace human activities.
%Digitalisation is generally beneficial, but this study brings awareness on what system engineers should prevent when re-thinking human-based processes. 

==> tables/table-subjects.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{ID} & \textbf{Researchers}             \\ \hline
RE\#1       & Social Science                   \\ \hline
RE\#2       & Agricultural Science              \\ \hline
RE\#3       & ICT and Software Engineering     \\ \hline
\rowcolor[HTML]{C0C0C0} 
\textbf{ID} & \textbf{Participants}            \\ \hline
RC\#1       & Coordinator of the RC            \\ \hline
TE\#1       & Field Technician of the RC       \\ \hline
TE\#2       & ICT Technician of the RC         \\ \hline
MU\#1       & Director of Municipalities Union \\ \hline
FA\#1       & Farmer and Interpreneur          \\ \hline
FA\#2       & Farmer and Interpreneur          \\ \hline
PR\#1       & IT Service Provider              \\ \hline
AS\#1       & Field Technician of Associations \\ \hline
AS\#2       & Field Technician of Associations \\ \hline
\end{tabular}
\caption{Interview Participants. \#RC1 performed two interviews.}
\label{tab:participants}
\end{table}
